Interactive Patch Filtering as Debugging Aid

It is widely recognized that program repair tools need to have a high precision to be useful, i.e., the generated patches need to have a high probability to be correct. However, it is fundamentally difficult to ensure the correctness of the patches, and many tools compromise other aspects of repair performance such as recall for an acceptable precision. In this paper we ask a question: can a repair tool with a low precision be still useful? To explore this question, we propose an interactive filtering approach to patch review, which filters out incorrect patches by asking questions to the developers. Our intuition is that incorrect patches can still help understand the bug. With proper tool support, the benefit outweighs the cost even if there are many incorrect patches. We implemented the approach as an Eclipse plugin tool, InPaFer, and evaluated it with a simulated experiment and a user study with 30 developers. The results show that our approach improve the repair performance of developers, with 62.5% more successfully repaired bugs and 25.3% less debugging time in average. In particular, even if the generated patches are all incorrect, the performance of the developers would not be significantly reduced, and could be improved when some patches provide useful information for repairing, such as the faulty location and a partial fix.

==> Discussion.tex <==
%!TEX root = ../InPaFer.tex
\section{Discussion} \label{section:discussion}


==> Introduction.tex <==
%!TEX root = ../InPaFer.tex
\section{Introduction} \label{section:introduction}
In the past decades, automatic program repair (APR) approaches~\cite{repair-survey2017,survey,kPAR-url,liu2019avatar,Wen2018ContextAwarePG,ISSTA18-SimFix,Xuan2016History,xiong-icse17,xuan2016nopol} have been proposed and make a significant progress. However, the bugs in real world are usually complicated and the ability of repair tools is limited. The recall of existing approaches is still very low, i.e, the recall of state-of-the-art tool, Hercules~\cite{DBLP:conf/icse/SahaSP19}, is only 13\%.

In addition, most of APR are test-based program repair. APR tools take a buggy program and test suits with at least a fail test as input, and automatically generate a set of patches which can make all test suits pass. However, a patch may be incorrect even if it can pass all test suites, because the test suites in real projects are usually weak~\cite{DBLP:conf/icse/XiongLZ0018}. The repair correctness cannot be guaranteed in theory. Therefore, APR tools generate a large number of incorrect patches, which will bring heavy burden to developers when reviewing the patches. 

In order to improve precision of APR, existing approaches may sacrifice the recall. Specifically, some tools may foucus on the bugs of specific type , such as ACS~\cite{xiong-icse17}, which only fixes condition error.
As a result, the recall of APR tools becomes lower. 
%However, even if the precision is improved, it seems still unrealistic to directly apply the auto-generated patches in production code because of developers' intrinsic resistance~\cite{DBLP:conf/sigsoft/TaoKKX14}.
%Some researches show that developers are less likely to accept the auto-generated patches because the patches are sometimes non-sensical~\cite{DBLP:conf/icse/KimNSK13}. Developers need to manually review the patches to make sure the patches are readable and maintainable~\cite{DBLP:conf/issta/FryLW12}.

Since existing APR approaches still need manual check and have a low recall, another idea is to improve the recall by integrating multiple APR tools. Because different APR tools target different types of bug, the recall of single tool is always lower than that of multiple tools. For example, the recall of state-of-the-art tool, Hercules~\cite{DBLP:conf/icse/SahaSP19}, is 13\%, while the recall of all existing APR tools, as far as we known, has achieve 24\% \todo{need to check the data}. 
However, the combined APR tools may generate many different patches for a bug and developers need to review more patches, which will bring more heavy burden to developers. Specially, Tao et al.~\cite{DBLP:conf/sigsoft/TaoKKX14} have found that when given low quality candidate patches, the developers' correctness will be affected deeply. 

In this paper, we propose an interactive repair approach which collects as many patches as possible from different APR tools to improve the recall. At same time, our approach adapts an interaction way to improve the efficiency of reviewing patches. Specifically, It first collects a set of plausible patches generated by existing APR tools and related to the bug. In this way, we can improve the recall of repair. As mentioned above, collecting many plausible patches will bring heavy burden to the developers. To address this challenge, for the candidate patches, we build constraints by collecting abundant of information, and question the developers whether the constraints should be satisfied. In this way, the developers can filter out or keep a group of patches at a time until the correct patches remain or all incorrect patches are filtered out. \ljj{need more specific?}

We have implemented our approach as an Eclipse plugin called \toolname, which stands for \textbf{In}teractive program repair by \textbf{Pa}tch \textbf{F}ilt\textbf{er}. In \toolname, we collected the patches from 13 program repair tools, which are available thus far. As for the constraints, we employed three kinds of constraints, including static code property (\method) and dynamic runtime information (\trace and \variable). 

We conducted two experiments on the Defects4J benchmark~\cite{just2014defects4j}. 
The simulated experiment evaluates the effectiveness of \toolname on 85 real bugs with simulated answers.
The results show that for about 49\% bugs, \toolname is able to filter out all incorrect patches or remain all correct patches within 3.5 questions on average. 
The user study evaluates the usefulness of \toolname in realistic scenarios, which involves 30 participants on 4 real-world bugs. We compared the efficiency and correctness of developers when debugging with \toolname (\fixwithtool) and with a set of patches (\fixwithPathes). In order to eliminate the effect of patches, we also conducted a experiment(\manualFix), in which the participants debug without any help.
The results show that \fixwithtool can reduce the debugging time by 28\% on average, and can improve the repair number by 11 (total 40), compared with \fixwithPathes.
Besides, \fixwithtool can reduce the debugging time by 25\% on average, and can improve the repair number by 15  (total 40), compared with \manualFix.

In addition, we also have some findings from the user study. When the candidate patch set has high quality and small number patches, \fixwithPathes can improve the effectiveness of \manualFix, otherwise the opposite. \fixwithtool can improve the effectiveness of \fixwithPathes, no matter how the quality and the number of candidate patches. However, when the candidate patch set contains low quality and a large number of patches, \fixwithtool shows more greater effectiveness. \ljj{copy from evaluation}


In summary, this paper makes the following contributions:
\begin{enumerate}
	\item An interactive program repair framework, which integrates the patches of existing APR tools.
	\item Three differential features of patch to build the interactive questions, and an interactive program repair tool with a graphic user interface, \toolname.
	\item A simulated experiment, which evaluates the effectiveness of \toolname in large real dataset.
	\item A user study, which investigates the usefulness of \toolname compared with manually repair with/without patches in real debugging tasks.
\end{enumerate}

The remainder of the paper is organized as follows. Section~\ref{section:runningexample} motivates our approach by an example. 
Section~\ref{section:approach} introduces the framework our approach. 
Section~\ref{section:implementation} illustrates our implementation in detail. 
Section~\ref{section:evaluation} evaluates the effectiveness of our approach on Defects4J, while Section~\ref{section:threats} and ~\ref{section:relatedwork} validates the threats and related work, respectively. 
Finally, Section~\ref{section:conclusion} concludes the paper.

==> Introduction_v1.tex <==
%!TEX root = ../InPaFer.tex
\section{Introduction} \label{section:introduction_v1}
In the past decades, automatic program repair (APR) approaches~\cite{repair-survey2017,survey,kPAR-url,liu2019avatar,Wen2018ContextAwarePG,ISSTA18-SimFix,Xuan2016History,xiong-icse17,xuan2016nopol} have been proposed and make a significant progress. Most of APR are test-based program repair. APR tools take a buggy program and test suits with  at least a fail test as input, and automatically generate a set of patches which can make all test suits pass. However, a patch may be incorrect even if it can pass all test suites, because the test suites in real projects are usually weak~\cite{DBLP:conf/icse/XiongLZ0018}. Therefore, the repair precision cannot be guaranteed in theory. 

In order to improve precision of APR, many approaches sacrifice the recall. Specifically, the precision of some APR tools can reaches from 70\% to 85\%, while the recall is less than 10\%, such as ACS~\cite{xiong-icse17} (73.8\%, 4.8\%) and CapGen~\cite{Wen2018ContextAwarePG} (84\%, 9.8\%). However, even if the precision is improved, it seems still unrealistic to directly apply the auto-generated patches in production code because of developers' intrinsic resistance~\cite{DBLP:conf/sigsoft/TaoKKX14}.
Some researches show that developers are less likely to accept the auto-generated patches because the patches are sometimes non-sensical~\cite{DBLP:conf/icse/KimNSK13}. Developers need to manually review the patches to make sure the patches are readable and maintainable~\cite{DBLP:conf/issta/FryLW12}.

\ljj{another version begin}
In the past decades, automatic program repair (APR) approaches~\cite{repair-survey2017,survey,kPAR-url,liu2019avatar,Wen2018ContextAwarePG,ISSTA18-SimFix,Xuan2016History,xiong-icse17,xuan2016nopol} have been proposed and make a significant progress. However, the bugs in real world are usually complicated and the ability of repair tools is limited. The recall of existing approaches is still very low, i.e, the recall of state-of-the-art tool, Hercules~\cite{DBLP:conf/icse/SahaSP19}, is only 13\%.

In addition, most of APR are test-based program repair. APR tools take a buggy program and test suits with at least a fail test as input, and automatically generate a set of patches which can make all test suits pass. However, a patch may be incorrect even if it can pass all test suites, because the test suites in real projects are usually weak~\cite{DBLP:conf/icse/XiongLZ0018}. The repair correctness cannot be guaranteed in theory. Therefore, APR tools generate a large number of incorrect patches, which will bring heavy burden to developers when reviewing the patches. 

In order to improve precision of APR, existing approaches may sacrifice the recall. Specifically, some tools may foucus on the bugs of specific type , such as ACS~\cite{xiong-icse17}, which only fixes condition error.
As a result, the recall of APR tools becomes lower. 
\ljj{another version end}

Since existing APR approaches still need manual check and have a low recall, another idea is to improve the recall by integrating multiple APR tools. Because different APR tools target different types of bug, the recall of single tool is always lower than that of multiple tools. For example, the recall of state-of-the-art tool, Hercules~\cite{DBLP:conf/icse/SahaSP19}, is 13\%, while the recall of all existing APR tools, as far as we known, has achieve 24\% \todo{need to check the data}. 
However, the combined APR tools may generate many  syntactic different patches for a bug and developers need to review more patches, which will bring more heavy burden to developers. Specially, Tao et al.~\cite{DBLP:conf/sigsoft/TaoKKX14} have found that when given low quality candidate patches, the developers' correctness will be affected deeply. 

In this paper, we propose an interactive repair approach which collects as many patches as possible and helps developers filter out the incorrect ones by questioning them. Specifically, It first collects a set of plausible patches generated by existing APR tools and related to the bug. In this way, we can improve the recall of repair.
As mentioned above, collecting many plausible patches will bring heavy burden to the developers. To address this challenge, for the candidate patches, we build constraints by collecting abundant of information, and question the developers whether the constraints should be satisfied. In this way, the developers can filter out or keep a group of patches at a time until the correct patches remain or all incorrect patches are filtered out. \ljj{need more specific?}

We have implemented our approach as an Eclipse plugin called \toolname, which stands for \textbf{In}teractive program repair by \textbf{Pa}tch \textbf{F}ilt\textbf{er}. In \toolname, we collected the patches from 13 program repair tools, which are available thus far. As for the constraints, we employed three kinds of constraints, including static code property (\method) and dynamic runtime information (\trace and \variable). 

We conducted two experiments on the Defects4J benchmark~\cite{just2014defects4j}. 
The simulated experiment evaluates the effectiveness of \toolname on 85 real bugs with simulated answers.
The results show that for about 49\% bugs, \toolname is able to filter out all incorrect patches or remain all correct patches within 3.5 questions on average. 
The user study evaluates the usefulness of \toolname in realistic scenarios, which involves 30 participants on 4 real-world bugs. We compared the efficiency and correctness of developers when debugging with \toolname (\fixwithtool) and with a set of patches (\fixwithPathes). In order to eliminate the effect of patches, we also conducted a experiment (\manualFix), in which the participants debug without any help. The results show that \fixwithtool can reduce the debugging time by 28\% on average, and can improve the repair number by 11 (total 40), compared with \fixwithPathes. Besides, \fixwithtool can reduce the debugging time by 25\% on average, and can improve the repair number by 15 (total 40), compared with \manualFix.

In addition, we also have some findings from the user study. When the candidate patch set has high quality and small number patches, \fixwithPathes can improve the effectiveness of \manualFix, otherwise the opposite. \fixwithtool can improve the effectiveness of \fixwithPathes, no matter how the quality and the number of candidate patches. However, when the candidate patch set contains low quality and a large number of patches, \fixwithtool shows more greater effectiveness. \ljj{copy from evaluation}


In summary, this paper makes the following contributions:
\begin{enumerate}
	\item An interactive program repair framework, which integrates the patches of existing APR tools.
	\item Three differential features of patch to build the interactive questions, and an interactive program repair tool with a graphic user interface, \toolname.
	\item A simulated experiment, which evaluates the effectiveness of \toolname in large real dataset.
	\item A user study, which investigates the usefulness of \toolname compared with manually repair with/without patches in real debugging tasks.
\end{enumerate}

The remainder of the paper is organized as follows. Section~\ref{section:runningexample} motivates our approach by an example. 
Section~\ref{section:approach} introduces the framework our approach. 
Section~\ref{section:implementation} illustrates our implementation in detail. 
Section~\ref{section:evaluation} evaluates the effectiveness of our approach on Defects4J, while Section~\ref{section:threats} and ~\ref{section:relatedwork} validates the threats and related work, respectively. 
Finally, Section~\ref{section:conclusion} concludes the paper.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts
		


==> RunningExample.tex <==
%!TEX root = ../InPaFer.tex
\section{Motivating Example} \label{section:runningexample}
This section motivates our approach using a real bug (Math41) from our experiment. The failing test case wants to test a method \textit{evaluate} in Math41, which involves 7 method invocations and 4 Java source files.
The assertion error will be triggered when given an array whose length more than 5.
We first collected 48 different patches from 3 APR tools. Then we built constraints for the patches and constructed a set of questions. As a result, we have 3 \method, 2 \variable and 28 \trace questions for Math41. 

We will illustrate the interaction by \trace questions. The developer first select a question, \textit{whether line 321 should be covered?} 
%This question corresponds 8 patches. 
As shown in figure~\ref{fig:codesnippet}, the developer will select ``No'' since it is easy to understand that the program should run the else branch. After answering the question, we will filter out all (8) patches corresponding to this question. As a result, there remain 40 candidate patches and 27 \trace questions. Similarly, the second question is querying the line 323, and the developer will select ``Yes''. Then, the candidate patch set will remain the 28 patches which correspond the second question. We will also set all questions which contains the same patches as ``Yes''. There remain 14 unanswered questions. Follow above steps, the developer need to answer 3 more questions and he/she will get the correct patch.

%\begin{lstlisting}[style=java,caption=A similar code
%snippet to the buggy one,label=lst:similar-code]
%if(last != null && last.getType() == Token.STRING){
%String propName = last.getString();
%return (propName.equals(methodName));
%}
%\end{lstlisting}

\begin{figure}[htb]
	\begin{lstlisting}[style=java,firstnumber=320]
    if (length == 1) {
        var = 0.0;
    } else if (length > 1) {
        Mean mean = new Mean();
    }
	\end{lstlisting}
	\caption{\label{fig:codesnippet} A code snippet from Math41}
\end{figure}
